Task Classification Model for Visual Fixation, Exploration, and Search

Yarbus' claim to decode the observer's task from eye movements has received mixed reactions. In this paper, we have supported the hypothesis that it is possible to decode the task. We conducted an exploratory analysis on the dataset by projecting features and data points into a scatter plot to visualize the nuance properties for each task. Following this analysis, we eliminated highly correlated features before training an SVM and Ada Boosting classifier to predict the tasks from this filtered eye movements data. We achieve an accuracy of 95.4% on this task classification problem and hence, support the hypothesis that task classification is possible from a user's eye movement data.

==> task_classification.tex <==
\section{Learning Task Classification}
In this task classification, we designed our study to classify four tasks given in the dataset. Focusing only on fixation data because (\textbf{Give reason here ...................................................................} We applied two classification algorithms: \textit{Support Vector Machines} and \textit{Adaptive Boosting} to learn from the ensemble of users that whether it is possible to classify the type of tasks being performed by just looking at the eye positioning of the users. By using the readings of \textit{LXPix, LYPix, LX href, LY href and LP} we could train classification models which can predict the type of task being performed, given the user's readings with time for any of the tasks. 

\subsection{Method: Data filtering}
This section explains the methodology applied in data filtering and training of the classifiers. Figure \ref{fig:system_layout} shows the block diagram of a task classification system. In this stage, all the data from every user and for every task are merged into a single large file. The time component is removed before training since the problem is to only predict the task category. We treat each timestamp readings as a single data point for training the classifier. After the files are merged, the Nan values are removed and the dataset is standardized by calculating the z-score for each column in the dataset. As shown in equation \ref{eq:zscore}, zscore is a method to convert a data distribution to standard normal by subtracting the mean $\mu$ and dividing by the standard deviation $\sigma$ for each column distribution in the dataset. We used zscore instead of Min Max normalization since zscore is more robust towards scaling the outliers. Now that the data is normalized, we shuffle the data points and split it to train, test and validation sets. The testing and validation sets contain about fifteen percent of the total data points each in our experiment. 
\begin{equation}
  z = \frac{x - \mu}{\sigma}
  \label{eq:zscore}
\end{equation}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{system_layout.png}
  \caption{Overview of the classifier trained for task prediction. A: Combine and shuffle the input files for training. B: Feed the task specific user file into the trained classifier. C: Classifier predicts the task.}
  \label{fig:system_layout}
\end{figure}

\subsection{Method: SVM classifier}
Support Vector Machines \cite{cortes1995support} is a famous classifier built to work with binary classification tasks. The main objective is to find the hyperplane which can separate the data points. The data points can be projected to higher dimensions for easier separation using the kernel function. For multiclass classification, one vs rest classification \cite{bottou1994comparison} technique is designed to use multiple binary classifiers to be trained for every label in the dataset \cite{hsu2002comparison}. Thus in this case, four different SVM classifiers are trained to each of the four tasks classification. The $i^{th}$ SVM is trained with the samples of $i^{th}$ class as positive and all others as negative. For the given training data $(x_{1}, y_{1}),...,(x_{l}, y_{l})$ with the labels in class from \textit{1} to \textit{k}, the multiclass SVM solves the problem shown in Equation \ref{eq:svm}. Minimizing the above function separates the positive and negative labels by maximum margin which can be controlled with the cost term C. In our experiment, the value of C = 700 gave the best results with training on 0.1\% of the datapoints. 


